Floating No More: Object-Ground Reconstruction from a Single Image

Recent advancements in 3D object reconstruction from single images have primarily focused on improving the accuracy of object shapes. Yet, these techniques often fail to accurately capture the inter-relation between the object, ground, and camera. As a result, the reconstructed objects often appear floating or tilted when placed on flat surfaces. This limitation significantly affects 3D-aware image editing applications like shadow rendering and object pose manipulation. To address this issue, we introduce ORG (Object Reconstruction with Ground), a novel task aimed at reconstructing 3D object geometry in conjunction with the ground surface. Our method uses two compact pixel-level representations to depict the relationship between camera, object, and ground. Experiments show that the proposed ORG model can effectively reconstruct object-ground geometry on unseen data, significantly enhancing the quality of shadow generation and pose manipulation compared to conventional single-image 3D reconstruction techniques.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/human-centric-depth-points.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[!t]
\vspace{2mm}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{\hskip 1mm}l@{\hskip 2mm}c@{\hskip 4mm}cc@{\hskip 3mm}cc}
\toprule
&  & \multicolumn{2}{c}{Depth Map\ \ \ \ \ \ } & \multicolumn{2}{c}{Point Clouds\ \ \ } \\ 
\cmidrule(r{2.5mm}){3-4}
\cmidrule(l{0mm}r{1mm}){5-6}
&  camera parameters  & \textbf{AbsRel}$\downarrow$ & $\boldsymbol{\delta_1}$$\uparrow$ & \textbf{LSIV}$\downarrow$ & \textbf{CD}$\downarrow$ \\ \midrule
{PIFu~\cite{saito2019pifu}} & \multirow{2}{*}{ortho. + const.}
    & 16.7     & 77.9     & 1.59     & 2.23     \\
{PIFuHD~\cite{saito2020pifuhd}}   & 
    & 14.1  & 83.1  & 1.27     & 1.85     \\
\midrule
{\textbf{\ourwork} (Ours)}   & our estimation
    & \textbf{10.3}  & \textbf{82.6}  & \textbf{1.21}     & \textbf{1.79}     \\
\bottomrule
\end{tabular}
}
\vspace{-1mm}
\caption{\ourwork perform slightly better in depth estimation and point cloud estimation tasks on 3DPeople dataset. And note that we also measures the object-ground relationship, and we are able to estimate for human images with more aggressive camera angles.  \textit{ortho.} stands for orthogonal projection, and \textit{const.} stands for heuristic constant. Numbers reported on 3DPeople dataset}
\label{table:human-centric-dp-pc}
\vspace{-2mm}
\end{table}
